Exponential escape efficiency of SGD from sharp minima in non-stationary regime

We show that stochastic gradient descent (SGD) escapes from sharp minima exponentially fast even before SGD reaches stationary distribution. SGD has been a de-facto standard training algorithm for various machine learning tasks. However, there still exists an open question as to why SGDs find highly generalizable parameters from non-convex target functions, such as the loss function of neural networks. An "escape efficiency" has been an attractive notion to tackle this question, which measures how SGD efficiently escapes from sharp minima with potentially low generalization performance. Despite its importance, the notion has the limitation that it works only when SGD reaches a stationary distribution after sufficient updates. In this paper, we develop a new theory to investigate escape efficiency of SGD with Gaussian noise, by introducing the Large Deviation Theory for dynamical systems. Based on the theory, we prove that the fast escape form sharp minima, named exponential escape, occurs in a non-stationary setting, and that it holds not only for continuous SGD but also for discrete SGD. A key notion for the result is a quantity called "steepness," which describes the SGD's stochastic behavior throughout its training process. Our experiments are consistent with our theory.

==> proofs/exit_time/main.tex <==
\section*{Exit time of Diffusion Process}
We consider the following diffusion process in $\R^d$, 
\begin{align}
\label{eq:diffusion_process}
\dot{x}_{t}^{}=-\nabla L\left(x_{t}\right)+\varepsilon D(x_{t})\dot{w}_{t},
\end{align}
where we assume the $\nabla L\left(\cdot\right)$ and $D(\cdot)$ are uniformly Lipschitz continuous.
We use $\varphi_t: \R \to \R^d$ to represent  trajectories of the process (i.e. realizations of $x_{t}$), which take time as an input and returns a position in $\R^d$.
We also write $\varphi\in \mathbf{C}_{T, x}\left(\mathbb{R}^{d}\right)$ to denote a trajectory with the time interval $[0,T]$ and $\varphi_0 = x$.
We consider an equilibrium point, $O$, and a closed domain around it, $B$, defined as follows.  
\begin{definition}[Domain $B$]
\leavevmode
\makeatletter
\@nobreaktrue
\makeatother
\begin{enumerate}
    \item $B\subseteq\R^d$ is a finite compact domain.
    \item $B$ contains a single asymptotically stable point $O$.
    \item $B$ is attracted to $O$.
    \item $\partial B$ is the boundary of $B$, which is continuous
    \item $(-\nabla L(x), n(x))<0$ holds for all $x \in \partial B$, where $n(x)$ is a normal vector of $\partial B$.
    \item $D(x)$ is positive definite for all $x\in B$.
\end{enumerate}
\end{definition}

We analyze the time for (\ref{eq:diffusion_process}) to exit from a domain $B$, called the \emph{exit time}.
\begin{definition}[Exit time]
$$
    \tau:=\min \left\{t: x_{t} \in \partial B\right\}
$$
\end{definition}


To analyze $\tau$, we introduce several important definitions.

\begin{definition}[Rate function]
$$
    S_{T}(\varphi) := \frac{1}{2} \int_{0}^{T}\left(\dot{\varphi}_t+\nabla L\left(\varphi_t\right)\right)^{T} D^{-1}\left(\varphi_t\right)\left(\dot{\varphi}_t+\nabla L\left(\varphi_t\right)\right) d t
$$
\end{definition}
Intuitively, $S_{T}(\varphi)$ means how steep $\varphi$ is on the train loss landscape, $L(\theta)$.
Mathematically, $S_{T}(\varphi)$ quantifies the distribution of $\varphi$ generated from (\ref{eq:diffusion_process}) in $B$ \citep{Dembo2010-fy,Freidlin2012-iz}.
More formally, from the Theorem 5.6.7 in \citep{Dembo2010-fy}, we can claim Lemma \ref{lemma:action_functional_1} and Lemma \ref{lemma:action_functional_2} regarding $S_{T}(\varphi)$.
\begin{lemma}
\label{lemma:action_functional_1}
For all $\delta,\zeta >0, \varphi \in \mathbf{C}_{T,x}\left(\R^{d}\right)$, there exists $ \varepsilon_\mathrm{RF1}(\varphi,\delta,\zeta)$ such that for all $\varepsilon\leq \varepsilon_\mathrm{RF1}(\varphi,\delta,\zeta)$,
$$
\mathrm{P}_{\varphi^\prime}\Big\{\varphi^\prime\in \mathbf{C}_{T,x}(\R^d)\mid \rho\left(\varphi^\prime, \varphi\right)<\delta\Big\} \geq \exp \left\{-\varepsilon^{-2}\left[S_{T}\left(\varphi\right)+\zeta\right]\right\},
$$
where $\rho(\varphi^\prime, \varphi)=\sup \left\{\|\varphi^\prime_t-\varphi_t\| \mid t \in [0,T]\right\}$.
\end{lemma}

\begin{lemma}
\label{lemma:action_functional_2}
Let $\Phi(s)=\left\{\varphi \in \mathbf{C}_{T,x}(\R^d)\mid S_{T}(\varphi) \leq s\right\}$. For all $\delta,\zeta,s >0$, there exists $\varepsilon_\mathrm{RF2}(s,\delta,\zeta)$ such that for all $\varepsilon\leq  \varepsilon_\mathrm{RF2}(s,\delta,\zeta)$,
$$
\mathrm{P}_{\varphi^\prime}\Big\{\varphi^\prime\in \mathbf{C}_{T,x}(\R^d) \mid \rho(\varphi^\prime, \Phi(s)) \geq \delta\Big\} \leq \exp \{-\varepsilon^{-2}(s-\zeta)\},
$$
where $\rho(\varphi^\prime, \Phi(s))=\inf \left\{\|\varphi^\prime-\varphi\| \mid \varphi \in \Phi(s)\right\}$.
\end{lemma}
Given $S_{T}(\varphi)$, we further define the following quantity.
\begin{definition}[Quasi-potential at $x$]
$$
    V( x):=\inf_{
                    \begin{array}{c}
                        \left\{\varphi \mid \scriptstyle \varphi_0=O, \varphi_T=x\right\}
                    \end{array}
                  }
    S_{T}(\varphi).
$$
\end{definition}
Here we claim the following theorem.
\begin{theorem}
\label{thm:basic_exit_time}
$$
\mathbb{E}_{x}\left[ \tau\right] =
\Theta\Big( \exp \left[\varepsilon^{-2}V_{0}\right]\Big)
$$
holds, where $V_0 := \min _{x^\prime \in \partial B} V(x^\prime)$
\end{theorem}
\begin{proof}


From Lemma \ref{lemma:exit_time_upper_bound}. and \ref{lemma:exit_time_lower_bound}., we can have
\begin{align}
    \mathbb{E}_{x}\left[ \tau\right]  = \Theta(\exp \left\{\varepsilon^{-2}V_{0}\right\}).
\end{align}

\end{proof}
\input{sections/exit_time/upper_bound/main}
\input{sections/exit_time/lower_bound/main}
\input{sections/exit_time/upper_bound/auxiliary_trajectories}


==> proofs/linear_algebra_max_min.tex <==

\begin{proof}[Proof of Lemma \ref{lemma:linear_algebra_max_of_min}]
We introduce several definitions only for this proof.
Supposing that we have a vector $x=\left(x_{1}, \ldots, x_{n}\right) \in \mathbb{R}^n$, $x^{\downarrow}$ and $x^{\uparrow}$ denote vectors whose coordinates are obtained by rearranging the numbers $x_{j}$ in decreasing order and in increasing order respectively, that is, $x^{\downarrow}=(x_{1}^{\downarrow}, \ldots, x_{n}^{\downarrow})$ and $x^{\uparrow}=(x_{1}^{\uparrow}, \ldots, x_{n}^{\uparrow})$, where $x_{1}^{\downarrow} \geq \cdots \geq x_{n}^{\downarrow}$ and $x_{1}^{\uparrow} \leq \cdots \leq x_{n}^{\uparrow}$.
Also, given $x, y \in \mathbb{R}^{n}$, we denote $x \prec y$, if 
\begin{align*}
\sum_{j=1}^{n} x_{j}^{\downarrow}=\sum_{j=1}^{n} y_{j}^{\downarrow}, \textrm{ and } \sum_{j=1}^{k} x_{j}^{\downarrow} \leq \sum_{j=1}^{k} y_{j}^{\downarrow} \textrm{ for } 1 \leq \forall k \leq n.
\end{align*}
For an $n \times n$ matrix $A$, $\lambda(A) = (\lambda_1(A),\lambda_2(A),...,\lambda_n(A))$.
Also, we define its elementwise logarithm $\log \lambda(A) = (\log \lambda_1(A),\log \lambda_2(A),...,\log \lambda_n(A))$.

Corollary I\hspace{-.1em}I\hspace{-.1em}I.4.6 in \citep{Bhatia1997-ib} claims that given two positive matrices $A$ and $B$, we have
\begin{align*}
\log \lambda^{\uparrow}(A) + \log \lambda^{\downarrow}(B) \prec \log \lambda(A B) \prec \log \lambda^{\downarrow}(A)+\log \lambda^{\downarrow}(B)
\end{align*}
Following the definition of $\prec$, the left part, $\log \lambda^{\uparrow}(A) + \log \lambda^{\downarrow}(B) \prec \log \lambda(A B)$, can be equivalently restated as
\begin{align*}
\sum_{j=1}^k\left\{\log \lambda^{\uparrow}(A) + \log \lambda^{\downarrow}(B) \right\}^{\downarrow}_j \leq \sum_{j=1}^k\left\{\log \lambda(A B)\right\}^{\downarrow}_j\textrm{ for } 1 \leq \forall k \leq n
\end{align*}
For the case $k = 1$, we have 
\begin{align*}
&\left\{\log \lambda^{\uparrow}(A) + \log \lambda^{\downarrow}(B) \right\}^{\downarrow}_1 \leq \left\{\log \lambda(A B)\right\}^{\downarrow}_1 \\
\Longleftrightarrow &\max_{1\leq i\leq n}\left\{\log \lambda_{n-i+1}(A)  + \log \lambda_i(B)\right\} \leq \log \lambda_\mathrm{max}(A B)
\end{align*}
Since $\max_{1\leq i\leq n}\left\{\log \lambda_{n-i+1}(A)  + \log \lambda_i(B) \right\} \geq \log \lambda_n(A)+\log \lambda_{1}(B) = \log \lambda_\mathrm{min}(A)+\log \lambda_\mathrm{max}(B)$ holds, we have $\log \lambda_\mathrm{min}(A)+\log \lambda_\mathrm{max}(B) \leq \log \lambda_\mathrm{max}(A B)$, or equivalently
\begin{align*}
\lambda_\mathrm{min}(A)\lambda_\mathrm{max}(B) \leq  \lambda_\mathrm{max}(A B).
\end{align*}

Since $ \lambda_\mathrm{max}(A) = 1/\lambda_\mathrm{min}(A^{-1})$ , we have
\begin{align*}
&\frac{1}{\lambda_\mathrm{max}(A^{-1})}\frac{1}{\lambda_\mathrm{min}(B^{-1})} \leq \frac{1}{\lambda_\mathrm{min}((AB)^{-1})}\\
\Longleftrightarrow\quad &\lambda_\mathrm{min}((AB)^{-1}) \leq \lambda_\mathrm{max}(A^{-1})\lambda_\mathrm{min}(B^{-1}).
\end{align*}
Since commuted matrices share eigenvalues, $\lambda_\mathrm{min}((AB)^{-1}) = \lambda_\mathrm{min}(B^{-1}A^{-1}) = \lambda_\mathrm{min}(A^{-1}B^{-1})$, we have
\begin{align*}
\lambda_\mathrm{min}(A^{-1}B^{-1}) \leq \lambda_\mathrm{max}(A^{-1})\lambda_\mathrm{min}(B^{-1}).
\end{align*}

\end{proof}


==> proofs/linear_algebra_min_min.tex <==
\begin{proof}[Proof of Lemma \ref{lemma:linear_algebra_min_of_min}]
$\lambda_{\max }(A)$ is equal to the spectral norm of $A$.
By the sub-multiplicative property of spectral norm, we obtain
\begin{align*}
   \lambda_{\max }(A) \lambda_{\max }(B) \geq \lambda_{\max }(A B) ,
\end{align*}
Therefore, since  $ \lambda_\mathrm{max}(A) = 1/\lambda_\mathrm{min}(A^{-1})$,
\begin{align*}
    & \lambda_{\max }(A^{-1}) \lambda_{\max }(B^{-1}) \geq \lambda_{\max }(A^{-1} B^{-1})\\ 
    \Longleftrightarrow\quad&  \lambda_{\max }(A^{-1}) \lambda_{\max }(B^{-1}) \geq\lambda_{\max }((A B)^{-1})\\
    \Longleftrightarrow\quad& \frac{1}{\lambda_{\min }(A) }\frac{1}{\lambda_{\min }(B)} \geq  \frac{1}{\lambda_{\min }(AB) }\\
    \Longleftrightarrow\quad& \lambda_{\min }(A B) \geq \lambda_{\min }(A) \lambda_{\min }(B).
\end{align*}
Then, we obtain the statement.
\end{proof}

==> proofs/sharpness_exit_time.tex <==

\textbf{Isotropic case $\mathrm{E}[\tau_\mathrm{isoSGD}]$:} We substitute $I$ to $C(\theta)$.
By the Jacobi equation (\ref{eq:jacobi_equation_display}) which is formally given by Theorem \ref{thm:jacobi_equation} in Appendix \ref{appendix:quasi_potential}, we have the following form for $\theta \in D$:
  \begin{align}
  \label{eq:neighbor_jacobian}
  \frac{1}{2}\nabla V(\theta)^\top  \nabla V(\theta)-\nabla L\left(\theta\right)^\top  \nabla V(\theta)=0.
  \end{align}
 We have $\nabla V(\theta) = 2 \nabla L(\theta)$ as a solution of (\ref{eq:neighbor_jacobian}).
  Given that $V(\theta^*) = 0$ by the definition of steepness and $L(\theta^*) = 0$ by Assumption \ref{assumption:unique}, we obtain $V(\theta) = 2 L(\theta) $ for $\theta \in D$.
  Therefore, we have
  \begin{align*}
      V_0 &= \min_{x\in\partial D}  2L(\theta) = \min_{x\in\partial D} 2\theta^\top H^* \theta = 2r^2\lambda.
  \end{align*}
  The second equality follows Assumption \ref{assumption:quadratic} and \ref{assumption:unique}.
  Combined with the fact (\ref{eq:exit_time_display}), which is formally shown in Theorem \ref{thm:basic_exit_time} in Appendix \ref{appendix:basic_exit_time}, we obtain the statement of Theorem \ref{thm:result} in the isotropic case.
  
 \textbf{Anisotropic case $\mathrm{E}[\tau_\mathrm{SGD}]$:} Similar to the isotropic case, the equation (\ref{eq:jacobi_equation_display}) (or Theorem \ref{thm:jacobi_equation}) gives 
\begin{align}
\label{eq:aniso_jacobian}
    \frac{1}{2}\nabla V(\theta)^\top{C(\theta)}^{\frac{1}{2}} \nabla V(\theta)-\nabla L\left(\theta\right)^\top \nabla V(\theta)=0.
\end{align}
$\nabla V(\theta) = 2 C(\theta)^{-\frac{1}{2}}\nabla L(\theta)$ is a solution of (\ref{eq:aniso_jacobian}). Then, by Assumption \ref{assumption:quadratic} and \ref{assumption:strong_covariance} , $\nabla V(\theta)$ is simply written as
\begin{align*}
        \nabla V(\theta)
        =2 H^{*-\frac{1}{2}}\nabla\left( \theta^\top H^*\theta\right) = 2 H^{*-\frac{1}{2}} 2H^*\theta= 4 {H^*}^{\frac{1}{2}}\theta.
\end{align*}
Given that $V(\theta^*) = 0$, we obtain $V(\theta) = \theta^\top  {H^*}^{\frac{1}{2}}\theta$ for $\theta \in D$.
Then, we rewrite $V_0$ is as
\begin{align}
\label{eq:V0_proof}
V_0 = 2r^2\lambda_\mathrm{min}({H^*}^{\frac{1}{2}}), 
\end{align}
Combined with (\ref{eq:exit_time_display}), or Theorem \ref{thm:basic_exit_time} in Appendix \ref{appendix:basic_exit_time}, we finish the proof of Theorem \ref{thm:result}.
